TABED: Test-Time Adaptive Ensemble Drafting for Robust Speculative Decoding in LVLMs

Speculative decoding (SD) has proven effective for accelerating LLM inference by quickly generating draft tokens and verifying them in parallel. However, SD remains largely unexplored for Large Vision-Language Models (LVLMs), which extend LLMs to process both image and text prompts. To address this gap, we benchmark existing inference methods with small draft models on 11 datasets across diverse input scenarios and observe scenario-specific performance fluctuations. Motivated by these findings, we propose Test-time Adaptive Batched Ensemble Drafting (TABED), which dynamically ensembles multiple drafts obtained via batch inference by leveraging deviations from past ground truths available in the SD setting. The dynamic ensemble method achieves an average robust walltime speedup of 1.74x over autoregressive decoding and a 5% improvement over single drafting methods, while remaining training-free and keeping ensembling costs negligible through parameter sharing. With its plug-and-play compatibility, we further enhance TABED by integrating advanced verification and alternative drafting methods. Code and custom-trained models are available at https://github.com/furiosa-ai/TABED.

==> acl/latex/main/exploring.tex <==
\section{Exploring Drafting Methods for LVLMs}
\label{sec:exploring}

% Re-written again by Byeongkeun Ahn
Since multimodal drafting does not consistently outperform text-only drafting in the preceding analysis (\cref{sec:study}), we investigate whether multimodal drafting can be improved. In this regard, we introduce and benchmark two alternative multimodal drafting schemes, \textit{pooled multimodal drafting} and \textit{caption drafting}, each equipped with a different mechanism to supply the draft model with visual information.

%\wonjun{...}
% Re-written by Byeongkeun Ahn
%As the preceding analysis is equivocal on whether multimodal information benefits drafting, we explore two variations of multimodal drafting. We find that they often but not always improve upon plain multimodal drafting. This hints us that \textit{combining} the variations discussed henceforth can be effective for building multimodal drafting schemes robust to diverse inputs, as we will show in \cref{sec:ensemble}. \wonjun{.......}

%In this section, we address several questions that arise during the drafting stage when applying speculative decoding to MLLMs, particularly about the necessity of images for drafting and the potential to substitute the image modality, considering that the draft model is imperfect and its performance can vary significantly across input scenarios.

\subsection{Pooled Multimodal Drafting}
%\subsection{\ba{Pooled Multimodal Drafting} How Necessary is the Image Modality for Drafting? \wonjun{...}}

% As mentioned earlier, the draft model is inherently imperfect and not effectively trained for long contexts.  => NEVER NEVER NEVER
What if we include image information in the draft model but compress its context? Previous works \citep{shang2024llava,chen2024image} show that although image tokens are more numerous than text tokens, their importance is relatively sparse, receiving meaningful attention only in certain layers. This sparsity has previously motivated the use of pooling to reduce the prefill size in LVLMs~\citep{mckinzie2024mm1methodsanalysis}. %Therefore, we can compress these image tokens, using this approach as a simple proxy for previous work aimed at reducing image prefill tokens.
% What if we include image information in the draft model but compress the context? According to previous studies\mj{Reference}, although image tokens are more numerous than text tokens, they are relatively sparse in importance—for example, receiving meaningful attention only in certain layers. So we can choose the way to compress these image tokens and make the way serve as the simplest proxy for previous works focusing on reducing image prefill tokens.
%\paragraph{Multimodal Drafting with Image-pooling}
%\subsection{Pooled Multimodal Drafting}
%\paragraph{Pooled Multimodal Drafting}
In line with this, we perform average pooling during inference to compress image information, preserving the 2D spatial structure of the image just before projector transformation into the text embedding space. %\minjae{Gone}The notation pool ($n$) indicates the number of visual tokens remaining from the original 576 tokens.
We employ a $2\times2$ pooling kernel that downsamples the total number of visual tokens from 576 to 144 as our default configuration (see \cref{app:pool} for experiments with various pooling rates).
Additionally, rather than just during inference, we also evaluate the performance of applying pooling from the instruction fine-tuning stage by training different models with various pooling rates in \cref{app:pool}.%Additionally, we applied image pooling from the instruction fine-tuning stage, obtaining different draft models for each pooling rate and conducted the same experiments (see Appendix). \wonjun{...}
% To compress image information, we performed average pooling in the $Z_v$ space \mj{To Wonjun: Llava model eq}, which maintains the 2D spatial information of the image just before it is transformed into the text representation space by the projector. We then create image prefill tokens by passing the pooled data through the projector $W$.The notation pool $n$ indicates the number of visual tokens remaining after pooling from the original 576 tokens per image. Since the compression is parameter-free, the cost is negligible. Additionally, we conducted experiments where, during the instruction fine-tuning stage (one of the two stages of training a pretrained LM into an MLLM), we trained the model while pooling the images at the same compression rates.

\paragraph{Experimental Results}

%From the perspective of block efficiency, for \standard{} datasets, the results after pooling were generally slightly worse than those without pooling. However, they still outperformed the text-only drafting for the most of datsets. This indicates that even the pooled visual tokens exhibit a certain level of image awareness.

\cref{tab:ensemble} shows the block efficiency results of pooled multimodal drafting. For \standard{} datasets, pooled multimodal drafting generally performs slightly worse than multimodal drafting. However, they still outperform text-only drafting for 4 out of 7 datasets. This indicates that even the pooled visual tokens exhibit a certain level of image awareness.

For \ood{} datasets, however, pooled multimodal drafting demonstrates significantly better performance than multimodal drafting and even better than text-only drafting. Pooling the visual tokens from 576 to just 144 significantly decreases the number of tokens by over 2k for OOD datasets requiring five input images, making pooled multimodal drafting more robust than original one.
%For \ood{} datasets, pooled multimodal drafting demonstrates significantly better performance than multimodal drafting and even better than text-only drafting. Pooling the visual tokens from 576 to just 144 significantly decreases the number of tokens by over 2k for OOD datasets requiring five input images, making pooled multimodal drafting—which has limited capacity to process long contexts—more robust. \minghao{this last sentence seems too convoluted}
%However, multimodal drafting with pooling demonstrated significantly better performance than multimodal drafting without pooling on a multi-image dataset with $n=5$. Pooling the tokens from 576 to just 144 significantly decreases the number of tokens, making multimodal drafting—which has limited capacity to process a large number of images—more robust. %In the case of multimodal drafting with a model fine-tuned through pooling, the trend was maintained while performance improved (see Appendix).%Table \ref{tab:explore}). To see the full results, refer Appendix.%~\ref{app:pool}.



%\input{tables/table_pooling}


% \begin{itemize}
%     \item \textbf{[EXPT]} Evaluation for LM/VLM tasks: multimodal (mm), pooled-$n$, text-only.
%     \item \textbf{[EXPT]} Fine-tuning results: maintained trends with improved performance (Appendix).
%     \item \textbf{[EXPT]} Top-$k$ image attention: Investigating whether issues arise due to the large number of tokens when attending to the prefill during the decoding stage, or if there is an inherent lack of multi-image prefill (modeling) capability (Appendix).
% \end{itemize}

%\subsection{\ba{Caption Drafting} Can We Replace Image Modality with Another one for Drafting? \wonjun{...}}
\subsection{Caption Drafting}

%\ba{In this section, we investigate whether it helps to augment the text-only draft model with image captions generated by another captioning model.}

% \subsection{Enhancing the Text-Only Draft Model through Caption Injection}

%Even without the image modality (i.e., text-only drafting), we observed substantial speed-ups (block efficiency), along with more robust performance compared to multimodal drafting. Therefore, is the image modality truly necessary for drafting?
We examine whether injecting image information into a text-only draft model improves block efficiency without direct image input. %\wonjun{imperfect draft model.. caption is helpful}
% In this section, we investigate whether injecting image information into a text-only draft model without providing image input can enhance block efficiency.%In this section, we investigate how injecting image information \textit{without} image input to the draft model. information into a text-only draft model can enhance block efficiency. 
%\paragraph{Caption Drafting}
One of the most straightforward ways to map images to the text modality is through captions. We employ a lightweight image captioning model to generate captions for each image, using these captions as input for the draft model instead of the images themselves. We use BLIP~\citep{li2022blip, li2023blip} and Florence~\citep{xiao2024florence} as captioning models whose latencies are shorter than the \prefill{} time of the target model. While we use Florence as our default model, BLIP performs comparably but much faster.
%We use BLIP~\citep{li2022blip, li2023blip} and Florence~\citep{xiao2024florence} as captioning models whose latencies are shorter than the \prefill{} time of the target model. While we use Florence as our default model, BLIP shows comparable performance with much higher efficiency.
%The choice of captioning model can be tailored to the size and prefill latency of the target model in deployment scenarios. 
% \minjae{caption: once in prefilling stage, processed in parallel with target model, V:P:D, amortization}
% The captioning model only needs to perform inference once during the \prefill{}.
The captioning model runs only once in parallel with the target model's \prefill{} stage. Technically, the latency from the captioning model's inference can be hidden within the prefill latency of the target model. Any minor latency due to factors like hardware variations is amortized across the entire decoding process (\cref{fig:timespan}), rendering it negligible.
% \minjae{The caption model runs only once in parallel with the prefilling stage of the target model, and technically, the latency induced by the inference of captioning model can be hided in the latency occuring in prefilling stage of target model. Any minor latency due to various factors as hardware caused by the captioning model's inference can be amortized across the entire decoding process (\cref{fig:timespan}), rendering it negligible.}
Details of the captioning models are in the \cref{app:caption}. %\ba{Details of the image captioning model can be found in Appendix.}%\cref{app:caption}.
% Details of the captioning models are in the \cref{app:cap_list,sec:app_cap_latency}. %\ba{Details of the image captioning model can be found in Appendix.}%\cref{app:caption}.
% One of the most straightforward methods to map images to the text modality is through captions. In our experimental setup, we employ a lightweight image captioning model to generate captions for each image and subsequently use these captions as input for the text-only draft model, rather than the images themselves. We used the BLIP~\citep{li2022blip, li2023blip} and Florence~\citep{xiao2024florence} models as lightweight image captioning models. The image captioning model only needs to perform inference once during the prefill, and its latency is shorter than the sum of the vision encoder processing and prefill time of the target model. Details of image captioning models are provided in \cref{app:caption}.

% \ba{What about moving the argument on the latency hiding of captioning models to a separate remark after experimental results?}


    %\input{figures/diagram}
    
\paragraph{Experimental Results}
%\wonjun{llama}
First, we consider the case of using LLaMA as a draft model. Since LLaMA lacks the ability to perceive the image modality, alternative input in text form, such as image captions, is essential for image comprehension. As shown in \cref{tab:ensemble}, caption drafting shows the best performance compared to text-only drafting across 6 out of 7 benchmark datasets and all OOD datasets.


%For LLaVA-1.5, as shown in Table~\ref{tab:ensemble}, caption drafting consistently outperforms text-only drafting across all datasets.
For LLaVA-1.5, as shown in \cref{tab:ensemble}, caption drafting achieves the best performance compared to text-only drafting across all benchmark datasets and OOD datasets.
Compared to multimodal drafting, caption-based drafting shows comparable performance on \standard{} datasets and significantly better performance on OOD datasets, indicating that caption-based drafting exhibits strong robustness similar to text-only drafting. \cref{fig:qual_1} shows a case where caption-based drafting achieves even better image comprehension than multimodal drafting, as the lightweight captioning model effectively extracts specific details like \textit{“Zane Crump.”}
%Furthermore, we conducted a detailed investigation comparing which tokens were successfully decoded (i.e., passed the target model's verification) and which failed to decode across different drafting methods. As shown in \cref{Venndiagram}, no single drafting method encompassed all the tokens correctly predicted by the others.
The full experimental results are in \cref{sec:app_cap_result}.

%As shown in \cref{tab:explore},  caption-based drafting showed improvements over text-only drafting from the perspective of block efficiency. \cref{fig:qual_1} shows that caption drafting outperforms text-only and multimodal drafting in image comprehension, as the lightweight captioning model extracts specific details like “Zane Crump.” Furthermore, we conducted a detailed investigation into which tokens each drafting method successfully decoded (i.e., passed the target model's verification) and which tokens it failed to decode. As shown in Figure~\ref{Venndiagram}, no single drafting method encompassed all the tokens correctly predicted by the others. Full experimental results of caption drafting are provided in Appendix.
%As shown in Figure~\ref{Venndiagram}, no single drafting method encompassed all the tokens correctly predicted by the others.
%\cref{app:caption}.



%\input{tables/table_caption}

%\input{figures/diagram}


% \section{Exploring Drafting Methods for MLLMs}


% \subsection{Enhancing the Text-Only Draft Model through Caption Injection}
% While the text-only draft model performs adequately in general, it exhibits a substantial performance decline, particularly in aspects requiring image comprehension, when compared to the multimodal draft model. In this section, we investigate how injecting image caption information into a text-only draft model can enhance block efficiency. 

% \paragraph{Experimental Settings}
% In our experimental setup, we employ a lightweight image captioning model to generate captions for each image and subsequently use these captions as input for the text-only draft model, rather than the images themselves. We used the BLIP series and Florence models as lightweight image captioning models. The image captioning model only needs to perform inference once during the prefill, and its latency is shorter than the prefill time of the target model. Details of lightweight image captioning models are provided in \cref{app:caption}.

% \paragraph{Experimental Results}
% \cref{tab:caption} shows ...

% Full experimental results of caption drafting are provided in \cref{app:caption}.
% \input{tables/table_caption}


% \subsection{Pooled Multimodal Drafting}

% \paragraph{Experimental Settings}
% In our experimental setup, we employ 2D average pooling on visual tokens. The notation pool (n) denotes that n represents the number of visual tokens remaining after the pooling operation.

% \paragraph{Experimental Results}

% \cref{tab:pooling} shows ...
% \input{tables/table_pooling}

% \input{figures/diagram}







\paragraph{Summary} As shown in \cref{VenndiagramWhole}, multimodal, text-only, caption, and pooled drafting methods demonstrate that each method offers unique advantages in drafting. 

\begin{figure}[!htb]
\centering
    \begin{subfigure}[b]{0.48\linewidth}
    \centering
            \resizebox{1\linewidth}{!}{%
\begin{tikzpicture}[font=\normalsize]
    \node at (-2.5, 2.5) {\large (a)};

    \begin{scope}[blend mode=screen]
        \fill[red!30]   (90:0.75) circle (1.5);
        \fill[blue!30] (210:0.75) circle (1.5);
        \fill[green!30]  (330:0.75) circle (1.5);
    \end{scope}


    \node at (90:2.5) {\textbf{Multimodal}};
    \node[rotate=-60] at (210:2.5) {\textbf{Text-only}};
    \node[rotate=60] at (330:2.5) {\textbf{Caption}};

    \node at (90:1.7) {2.5\%}; %M
    \node at (210:1.7) {1.1\%}; %T
    \node at (330:1.7) {2.7\%}; %C

    \node at (0:0) {47.1\%}; %MTC

    \node at (30:1.2) {1.4\%}; %MC
    \node at (150:1.2) {1.9\%}; %MT
    \node at (270:1.2) {2.3\%}; %TC
\end{tikzpicture}
}
\label{Venndiagram}
\end{subfigure}
\hfill
    \begin{subfigure}[b]{0.48\linewidth}
        \centering
            \resizebox{1\linewidth}{!}{%
\begin{tikzpicture}[font=\normalsize]
    \node at (-2.5, 2.5) {\large (b)};

    \draw[black, ultra thick] (90:0.75) circle (1.5);
    \draw[black, ultra thick] (210:0.75) circle (1.5);
    \draw[black, ultra thick] (330:0.75) circle (1.5);


    \begin{scope}[blend mode=screen]
        \fill[red!30]   (90:0.75) circle (1.5);
        \fill[blue!30] (210:0.75) circle (1.5);
        \fill[green!30]  (330:0.75) circle (1.5);
    \end{scope}


    \node at (90:2.5) {\textbf{Multimodal}};
    \node[rotate=-60] at (210:2.5) {\textbf{Text-only}};
    \node[rotate=60] at (330:2.5) {\textbf{Caption}};

    \node at (90:1.7) {different}; %M
    \node at (210:1.7) {“}; %T
    \node at (330:1.7) {Crump}; %C

    \node at (0:0) {\textbf{\huge Ensemble}}; %MTC

    \node at (30:1.2) {$\cdots$}; %MC
    \node at (150:1.2) {$\cdots$}; %MT
    \node at (270:1.2) {$\cdots$}; %TC
\end{tikzpicture}
}
%\caption{Venn diagram of the accepted tokens for each drafting method on \cref{fig:qual_1}}
\label{Venndiagram2}
\end{subfigure}
\captionsetup{skip=-8pt}
\caption{Venn diagrams showing (a) the acceptance rates of each drafting method on the ChartQA dataset and (b) examples of tokens accepted by one method but not by the others in \cref{fig:qual_1}.}% The ensemble method can draft all tokens in $\lbrace$different, “ , Crump$\rbrace$, whereas each individual method would miss some of them.}
\label{VenndiagramWhole}
\end{figure}


==> acl/latex/tables/table_app_caption.tex <==
\begin{table*}[h]
\centering
\sisetup{table-auto-round}
\resizebox{1.0\textwidth}{!}{% 
\begin{tabular}{lrl|ccccccc||cc}
\toprule
\multicolumn{3}{c|}{Draft Model} & \multicolumn{7}{c||}{\titlecap{\standard{} datasets}} & \multicolumn{2}{c}{\titlecap{\ood{} datasets}} \\%&$n=1$&$n=2$&$n=5$ \\
\cmidrule(lr){1-3}\cmidrule(lr){4-10}\cmidrule(lr){11-12}%\cmidrule(lr){12-12}\cmidrule(lr){13-13}\cmidrule(lr){14-14}
Type & Size & Method  & ChartQA \citep{masry2022chartqa} & TextVQA \citep{singh2019towards} & VQAv2 \citep{goyal2017making}& HBench \citep{guan2024hallusionbench}& Spot \citep{jhamtani2018learning}& WebQA \citep{chang2022webqa}& MB \citep{zhang2024magicbrush}& PSV \citep{li2019storygan}& VIST \citep{huang2016visual}\\
\midrule
 \multirow{18}{*}{\shortstack[l]{LLaVA-1.5}}  &  \multirow{18}{*}{68M}  &  M  &  2.24 &  2.12 &  2.26 &  2.39 &  2.34 &  2.51 &  1.96 &  1.19 &  1.16 \\
  &    &  T  &  2.22 &  2.03 &  2.20 &  2.34 &  2.27 &  2.77 &  2.34 &  2.05 &  2.05 \\
  &    &  C (F-2-C)  &  2.28 &  2.08 &  2.24 &  2.41 &  2.31 &  2.77 &  2.36 &  2.08 &  2.10 \\
  &    &  C (F-2-MDC)  &  2.27 &  2.11 &  2.26 &  \secondbest{2.44} &  2.28 &  2.74 &  2.36 &  2.10 &  2.11 \\
  &    &  C (BLIP)  &  2.23 &  2.02 &  2.23 &  2.40 &  2.28 &  2.75 &  2.37 &  \best{2.12} &  2.10 \\
  &    &  C (BLIP-2)  &  2.25 &  2.07 &  2.23 &  2.37 &  2.30 &  2.78 &  2.37 &  2.09 &  2.12 \\
  &    &  MC (F-2-C)  &  \cellcolor{mymax}\secondbest{2.30} &  \cellcolor{mymax}\best{2.17} &  \cellcolor{mymax}\secondbest{2.29} &  \cellcolor{mymax}2.42 &  \cellcolor{mymax}2.39 &  2.74 &  2.35 &  1.99 &  1.93 \\
  &    &  MC (F-2-MDC)  &  \cellcolor{mymax}\best{2.31} &  \cellcolor{mymax}\best{2.17} &  \cellcolor{mymax}\best{2.30} &  \cellcolor{mymax}\best{2.46} &  \cellcolor{mymax}2.38 &  2.73 &  2.34 &  1.99 &  1.96 \\
   &    &  MC (BLIP)  &  \cellcolor{mymax}2.27 &  2.11 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.42 &  \cellcolor{mymax}2.37 &  2.72 &  2.35 &  2.00 &  1.94 \\
  &    &  MC (BLIP-2)  &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.15 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.40 &  \cellcolor{mymax}2.39 &  2.75 &  2.34 &  1.98 &  1.95 \\
  &    &  MTC (F-2-C)  &  \cellcolor{mymax}2.29 &  \cellcolor{mymax}2.15 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.41 &  \cellcolor{mymax}\best{2.41} &  \cellcolor{mymax}2.79 &  \cellcolor{mymax}\secondbest{2.40} &  \cellcolor{mymax}2.08 &  2.06 \\
  &    &  MTC (F-2-MDC)  &  \cellcolor{mymax}2.29 &  \cellcolor{mymax}2.15 &  \cellcolor{mymax}\secondbest{2.29} &  \cellcolor{mymax}\secondbest{2.44} &  \cellcolor{mymax}\secondbest{2.40} &  \cellcolor{mymax}2.79 &  \cellcolor{mymax}\best{2.41} &  2.09 &  2.08 \\
   &    &  MTC (BLIP)  &  \cellcolor{mymax}2.26 &  2.11 &  \cellcolor{mymax}2.27 &  \cellcolor{mymax}2.41 &  \cellcolor{mymax}2.38 &  \cellcolor{mymax}2.78 &  \cellcolor{mymax}2.39 &  2.05 &  2.05 \\
  &    &  MTC (BLIP-2)  &  \cellcolor{mymax}2.26 &  \cellcolor{mymax}2.14 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.40 &  \cellcolor{mymax}2.39 &  \cellcolor{mymax}\best{2.81} &  \cellcolor{mymax}\secondbest{2.40} &  2.06 &  2.06 \\
   &    &  MTCP (F-2-C)  &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.16 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.41 &  \cellcolor{mymax}\secondbest{2.40} &  \cellcolor{mymax}2.78 &  \cellcolor{mymax}2.39 &  \cellcolor{mymax}2.10 &  \cellcolor{mymax}\secondbest{2.13} \\
  &    &  MTCP (F-2-MDC)  &  \cellcolor{mymax}2.29 &  \cellcolor{mymax}2.15 &  \cellcolor{mymax}\secondbest{2.29} &  2.43 &  \cellcolor{mymax}2.39 &  \cellcolor{mymax}2.79 &  \cellcolor{mymax}\secondbest{2.40} &  \cellcolor{mymax}\best{2.12} &  \cellcolor{mymax}\best{2.15} \\
   &    &  MTCP (BLIP)  &  \cellcolor{mymax}2.26 &  2.11 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.41 &  \cellcolor{mymax}2.39 &  \cellcolor{mymax}2.78 &  \cellcolor{mymax}2.39 &  2.08 &  \cellcolor{mymax}\secondbest{2.13} \\
  &    &  MTCP (BLIP-2)  &  \cellcolor{mymax}2.26 &  \cellcolor{mymax}2.14 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.40 &  \cellcolor{mymax}2.39 &  \cellcolor{mymax}\secondbest{2.80} &  \cellcolor{mymax}2.39 &  \cellcolor{mymax}2.09 &  \cellcolor{mymax}\secondbest{2.13} \\
\bottomrule
\end{tabular}
}
\caption{Evaluations of block efficiency for various image captioning models and prompts under single-method and ensemble drafting scenarios. Results of IbED are \hlc[gray!15]{highlighted} when they show the best performance among all constituent methods (e.g., when MC performs best compared to M and C). Overall, Florence-2 demonstrates slightly better efficacy than BLIP and BLIP-2. The efficacy of Florence-2 captions can often be improved by the use of the more detailed captions (MDC) prompt compared to the default captions (C) prompt. Note that the benefits in block efficiency must be carefully weighed against the extra latency incurred by the generation of longer captions.}
% \caption{\ba{Evaluations of block efficiency for various image captioning models and prompts under single-method and ensemble drafting scenarios. Results of IbED are \hlc[gray!15]{highlighted} when they show the best performance among all constituent methods (e.g., when MC performs best compared to M and C). Overall, Florence-2 demonstrates slightly better efficacy than BLIP and BLIP-2. The efficacy of Florence-2 captions can often be improved by the use of the more detailed captions (MDC) prompt compared to the default captions (C) prompt. Note that the benefits in block efficiency must be carefully weighed against the extra latency incurred by the generation of longer captions.} \wonjun{merge please}}
%\ba{Evaluations of block efficiency for various image captioning models and prompts under single-method drafting and ensemble drafting.} \ba{Maybe separate the two tables and remove this caption?}  ... Block efficiency results for various image captioning models. \ba{The efficacy of Florence captions in enhancing the block efficiency can often be improved by the use of the more detailed captions (MDC) prompt compared to the default captions (C) prompt. Note that the benefits in block efficiency must be carefully weighed against the extra latency incurred by the generation of longer captions. Overall, the Florence models demonstrate slightly better efficacy than BLIP and BLIP-2.} Block efficiency results of ensemble drafting with detailed captions. \ba{Comparison of two captioning prompts under ensemble drafting. Results of IbED are \hlc[gray!15]{highlighted} when they show the best performance among all constituent methods (e.g., when MC performs best compared to M and C). Based on the result, we make the default captions (C) prompt our default choice for other experiments.}\wonjun{merge please}
\label{tab:app_cap}
\end{table*}




\begin{comment}
\begin{table*}[ht]
\centering
\begin{subtable}[t]{\textwidth}
\centering
\resizebox{\textwidth}{!}{
\sisetup{table-auto-round}
\begin{tabular}{lrl|ccccccc||cc}
\toprule
\multicolumn{3}{c|}{Draft Model} & \multicolumn{7}{c||}{\titlecap{\standard{} datasets}} & \multicolumn{2}{c}{\titlecap{\ood{} datasets}} \\%&$n=1$&$n=2$&$n=5$ \\
\cmidrule(lr){1-3}\cmidrule(lr){4-10}\cmidrule(lr){11-12}%\cmidrule(lr){12-12}\cmidrule(lr){13-13}\cmidrule(lr){14-14}
Type & Size & Method  & ChartQA \citep{masry2022chartqa} & TextVQA \citep{singh2019towards} & VQAv2 \citep{goyal2017making}& HBench \citep{guan2024hallusionbench}& Spot \citep{jhamtani2018learning}& WebQA \citep{chang2022webqa}& MB \citep{zhang2024magicbrush}& PSV \citep{li2019storygan}& VIST \citep{huang2016visual}\\
\midrule
\multirow{6}{*}{\shortstack[l]{LLaVA-1.5}} & \multirow{6}{*}{68M} & Multimodal & 2.24 & \best{2.12} & \best{2.26} & 2.39 & \best{2.34} & 2.51 & 1.96 & 1.19 & 1.16  \\%&\cellcolor{mysilver}2.25 & 2.26 & 1.17 \\
 &  & Text-only & 2.22 & 2.03 & 2.20 & 2.34 & 2.27 & \secondbest{2.77} & 2.34 & 2.05 & 2.05 \\%& 2.20 & 2.25 & 2.05 \\
 &  & Caption (F-2-C) & \best{2.28} & 2.08 & 2.24 & \secondbest{2.41} & \secondbest{2.31} & \secondbest{2.77} & 2.36 & 2.08 & 2.10 \\%& \cellcolor{mysilver}2.25 & \cellcolor{mygold}2.30 & 2.09 \\
 &  & Caption (F-2-MDC) & \secondbest{2.27} & \secondbest{2.11} & \best{2.26} & \best{2.44} & 2.28 & 2.74 & 2.36 & \secondbest{2.10} & \secondbest{2.11} \\%& \cellcolor{mygold}2.27 & \cellcolor{mysilver}2.29 & \cellcolor{mysilver}2.10 \\
 &  & Caption (BLIP) & 2.23 & 2.02 & 2.23 & 2.40 & 2.28 & 2.75 & \best{2.37} & \best{2.12} & 2.10 \\
 &  & Caption (BLIP-2) & 2.25 & 2.07 & 2.23 & 2.37 & 2.30 & \best{2.78} & \best{2.37} & 2.09 & \best{2.12} \\
\bottomrule
\end{tabular}
}
\caption{}
\label{tab:app_cap1}
\end{subtable}
\medskip

\begin{subtable}[t]{\textwidth}
\centering
\resizebox{\textwidth}{!}{
\sisetup{table-auto-round}
\begin{tabular}{lrl|ccccccc||cc}
\toprule
\multicolumn{3}{c|}{Draft Model} & \multicolumn{7}{c||}{\titlecap{\standard{} datasets}} & \multicolumn{2}{c}{\titlecap{\ood{} datasets}} \\%&$n=1$&$n=2$&$n=5$ \\
\cmidrule(lr){1-3}\cmidrule(lr){4-10}\cmidrule(lr){11-12}%\cmidrule(lr){12-12}\cmidrule(lr){13-13}\cmidrule(lr){14-14}
Type & Size & Method  & ChartQA \citep{masry2022chartqa} & TextVQA \citep{singh2019towards} & VQAv2 \citep{goyal2017making}& HBench \citep{guan2024hallusionbench}& Spot \citep{jhamtani2018learning}& WebQA \citep{chang2022webqa}& MB \citep{zhang2024magicbrush}& PSV \citep{li2019storygan}& VIST \citep{huang2016visual}\\
\midrule
 \multirow{18}{*}{\shortstack[l]{LLaVA-1.5}}  &  \multirow{18}{*}{68M}  &  M  &  2.24 &  2.12 &  2.26 &  2.39 &  2.34 &  2.51 &  1.96 &  1.19 &  1.16 \\
  &    &  T  &  2.22 &  2.03 &  2.20 &  2.34 &  2.27 &  2.77 &  2.34 &  2.05 &  2.05 \\
  &    &  C (F-2-C)  &  2.28 &  2.08 &  2.24 &  2.41 &  2.31 &  2.77 &  2.36 &  2.08 &  2.10 \\
  &    &  C (F-2-MDC)  &  2.27 &  2.11 &  2.26 &  \secondbest{2.44} &  2.28 &  2.74 &  2.36 &  2.10 &  2.11 \\
  &    &  C (BLIP)  &  2.23 &  2.02 &  2.23 &  2.40 &  2.28 &  2.75 &  2.37 &  \best{2.12} &  2.10 \\
  &    &  C (BLIP-2)  &  2.25 &  2.07 &  2.23 &  2.37 &  2.30 &  2.78 &  2.37 &  2.09 &  2.12 \\
  &    &  MC (F-2-C)  &  \cellcolor{mymax}\secondbest{2.30} &  \cellcolor{mymax}\best{2.17} &  \cellcolor{mymax}\secondbest{2.29} &  \cellcolor{mymax}2.42 &  \cellcolor{mymax}2.39 &  2.74 &  2.35 &  1.99 &  1.93 \\
  &    &  MC (F-2-MDC)  &  \cellcolor{mymax}\best{2.31} &  \cellcolor{mymax}\best{2.17} &  \cellcolor{mymax}\best{2.30} &  \cellcolor{mymax}\best{2.46} &  \cellcolor{mymax}2.38 &  2.73 &  2.34 &  1.99 &  1.96 \\
   &    &  MC (BLIP)  &  \cellcolor{mymax}2.27 &  2.11 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.42 &  \cellcolor{mymax}2.37 &  2.72 &  2.35 &  2.00 &  1.94 \\
  &    &  MC (BLIP-2)  &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.15 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.40 &  \cellcolor{mymax}2.39 &  2.75 &  2.34 &  1.98 &  1.95 \\
  &    &  MTC (F-2-C)  &  \cellcolor{mymax}2.29 &  \cellcolor{mymax}2.15 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.41 &  \cellcolor{mymax}\best{2.41} &  \cellcolor{mymax}2.79 &  \cellcolor{mymax}\secondbest{2.40} &  \cellcolor{mymax}2.08 &  2.06 \\
  &    &  MTC (F-2-MDC)  &  \cellcolor{mymax}2.29 &  \cellcolor{mymax}2.15 &  \cellcolor{mymax}\secondbest{2.29} &  \cellcolor{mymax}\secondbest{2.44} &  \cellcolor{mymax}\secondbest{2.40} &  \cellcolor{mymax}2.79 &  \cellcolor{mymax}\best{2.41} &  2.09 &  2.08 \\
   &    &  MTC (BLIP)  &  \cellcolor{mymax}2.26 &  2.11 &  \cellcolor{mymax}2.27 &  \cellcolor{mymax}2.41 &  \cellcolor{mymax}2.38 &  \cellcolor{mymax}2.78 &  \cellcolor{mymax}2.39 &  2.05 &  2.05 \\
  &    &  MTC (BLIP-2)  &  \cellcolor{mymax}2.26 &  \cellcolor{mymax}2.14 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.40 &  \cellcolor{mymax}2.39 &  \cellcolor{mymax}\best{2.81} &  \cellcolor{mymax}\secondbest{2.40} &  2.06 &  2.06 \\
   &    &  MTCP (F-2-C)  &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.16 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.41 &  \cellcolor{mymax}\secondbest{2.40} &  \cellcolor{mymax}2.78 &  \cellcolor{mymax}2.39 &  \cellcolor{mymax}2.10 &  \cellcolor{mymax}\secondbest{2.13} \\
  &    &  MTCP (F-2-MDC)  &  \cellcolor{mymax}2.29 &  \cellcolor{mymax}2.15 &  \cellcolor{mymax}\secondbest{2.29} &  2.43 &  \cellcolor{mymax}2.39 &  \cellcolor{mymax}2.79 &  \cellcolor{mymax}\secondbest{2.40} &  \cellcolor{mymax}\best{2.12} &  \cellcolor{mymax}\best{2.15} \\
   &    &  MTCP (BLIP)  &  \cellcolor{mymax}2.26 &  2.11 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.41 &  \cellcolor{mymax}2.39 &  \cellcolor{mymax}2.78 &  \cellcolor{mymax}2.39 &  2.08 &  \cellcolor{mymax}\secondbest{2.13} \\
  &    &  MTCP (BLIP-2)  &  \cellcolor{mymax}2.26 &  \cellcolor{mymax}2.14 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.40 &  \cellcolor{mymax}2.39 &  \cellcolor{mymax}\secondbest{2.80} &  \cellcolor{mymax}2.39 &  \cellcolor{mymax}2.09 &  \cellcolor{mymax}\secondbest{2.13} \\
\bottomrule
\end{tabular}
}
\caption{Block efficiency results of ensemble drafting with detailed captions. \ba{Comparison of two captioning prompts under ensemble drafting. Results of IbED are \hlc[gray!15]{highlighted} when they show the best performance among all constituent methods (e.g., when MC performs best compared to M and C). Based on the result, we make the default captions (C) prompt our default choice for other experiments.}}
\label{tab:app_cap2}
\end{subtable}
\caption{\ba{Evaluations of block efficiency for various image captioning models and prompts under single-method drafting and ensemble drafting.} \ba{Maybe separate the two tables and remove this caption?}  ... Block efficiency results for various image captioning models. \ba{The efficacy of Florence captions in enhancing the block efficiency can often be improved by the use of the more detailed captions (MDC) prompt compared to the default captions (C) prompt. Note that the benefits in block efficiency must be carefully weighed against the extra latency incurred by the generation of longer captions. Overall, the Florence models demonstrate slightly better efficacy than BLIP and BLIP-2.} Block efficiency results of ensemble drafting with detailed captions. \ba{Comparison of two captioning prompts under ensemble drafting. Results of IbED are \hlc[gray!15]{highlighted} when they show the best performance among all constituent methods (e.g., when MC performs best compared to M and C). Based on the result, we make the default captions (C) prompt our default choice for other experiments.}\wonjun{merge please}}
%\label{tab:1_all}
\end{table*}
\end{comment}










==> acl/latex/tables/table_app_ensemble.tex <==
\begin{table*}[h]
\centering
\sisetup{table-auto-round}
\resizebox{1.0\textwidth}{!}{% 
\begin{tabular}{lrl|ccccccc||cc}
\toprule
\multicolumn{3}{c|}{Draft Model} & \multicolumn{7}{c||}{\titlecap{\standard{} datasets}} & \multicolumn{2}{c}{\titlecap{\ood{} datasets}} \\%&$n=1$&$n=2$&$n=5$ \\
\cmidrule(lr){1-3}\cmidrule(lr){4-10}\cmidrule(lr){11-12}%\cmidrule(lr){12-12}\cmidrule(lr){13-13}\cmidrule(lr){14-14}
Type & Size & Method (Weights) & ChartQA \citep{masry2022chartqa} & TextVQA \citep{singh2019towards} & VQAv2 \citep{goyal2017making}& HBench \citep{guan2024hallusionbench}& Spot \citep{jhamtani2018learning}& WebQA \citep{chang2022webqa}& MB \citep{zhang2024magicbrush}& PSV \citep{li2019storygan}& VIST \citep{huang2016visual}\\
\midrule
\multirow{24}{*}{\shortstack[l]{LLaVA-1.5}}  &  \multirow{24}{*}{68M}  &  M  &  2.24 &  2.12 &  2.26 &  2.39 &  2.34 &  2.51 &  1.96 &  1.19 &  1.16 \\
  &    &  T  &  2.22 &  2.03 &  2.20 &  2.34 &  2.27 &  2.77 &  2.34 &  2.05 &  2.05 \\
  &    &  C  &  2.28 &  2.08 &  2.24 &  2.41 &  2.31 &  2.77 &  2.36 &  \secondbest{2.08} &  \secondbest{2.10} \\
  &    &  P  &  2.23 &  2.08 &  2.26 &  2.36 &  2.23 &  2.73 &  2.27 &  2.07 &  2.09 \\
  &    &  MT (1:1)  &  \cellcolor{mymax}2.26 &  \cellcolor{mymax}2.13 &  \cellcolor{mymax}2.27 &  \cellcolor{mymax}2.39 &  \cellcolor{mymax}2.40 &  2.75 &  \cellcolor{mymax}2.37 &  1.94 &  1.91 \\
  &    &  MT (2:1)  &  \cellcolor{mymax}2.26 &  \cellcolor{mymax}2.13 &  \cellcolor{mymax}\secondbest{2.29} &  \cellcolor{mymax}2.39 &  \cellcolor{mymax}2.40 &  2.69 &  2.29 &  1.76 &  1.69 \\
  &    &  MT (3:1)  &  \cellcolor{mymax}2.26 &  \cellcolor{mymax}2.13 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.40 &  \cellcolor{mymax}2.38 &  2.65 &  2.21 &  1.63 &  1.54 \\
  &    &  MT (4:1)  &  \cellcolor{mymax}2.26 &  \cellcolor{mymax}2.14 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.40 &  \cellcolor{mymax}2.36 &  2.64 &  2.16 &  1.54 &  1.45 \\
  &    &  MC (1:1)  &  \cellcolor{mymax}\best{2.30} &  \cellcolor{mymax}\best{2.17} &  \cellcolor{mymax}\secondbest{2.29} &  \cellcolor{mymax}\best{2.42} &  \cellcolor{mymax}2.39 &  2.74 &  2.35 &  1.99 &  1.93 \\
  &    &  MC (2:1)  &  \cellcolor{mymax}\best{2.30} &  \cellcolor{mymax}\best{2.17} &  \cellcolor{mymax}\best{2.30} &  \cellcolor{mymax}2.41 &  \cellcolor{mymax}2.39 &  2.70 &  2.27 &  1.80 &  1.71 \\
  &    &  MC (3:1)  &  \cellcolor{mymax}2.29 &  \cellcolor{mymax}2.16 &  \cellcolor{mymax}\secondbest{2.29} &  2.40 &  \cellcolor{mymax}2.38 &  2.66 &  2.20 &  1.66 &  1.56 \\
  &    &  MC (4:1)  &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.16 &  \cellcolor{mymax}\secondbest{2.29} &  2.40 &  \cellcolor{mymax}2.37 &  2.64 &  2.16 &  1.56 &  1.46 \\
  &    &  MTC (1:1:1)  &  \cellcolor{mymax}2.29 &  \cellcolor{mymax}2.15 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.41 &  \cellcolor{mymax}\best{2.41} &  \cellcolor{mymax}\best{2.79} &  \cellcolor{mymax}\best{2.40} &  \cellcolor{mymax}\secondbest{2.08} &  2.06 \\
  &    &  MTC (2:1:1)  &  \cellcolor{mymax}2.29 &  \cellcolor{mymax}\best{2.17} &  \cellcolor{mymax}\secondbest{2.29} &  \cellcolor{mymax}\best{2.42} &  \cellcolor{mymax}\best{2.41} &  2.73 &  \cellcolor{mymax}2.38 &  1.99 &  1.96 \\
  &    &  MTC (3:1:1)  &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}\best{2.17} &  \cellcolor{mymax}\secondbest{2.29} &  \cellcolor{mymax}2.41 &  \cellcolor{mymax}2.39 &  2.69 &  2.34 &  1.90 &  1.83 \\
  &    &  MTC (4:1:1)  &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.16 &  \cellcolor{mymax}\secondbest{2.29} &  2.40 &  \cellcolor{mymax}2.39 &  2.67 &  2.29 &  1.80 &  1.71 \\
   &    &  MTP (1:1:1)  &  \cellcolor{mymax}2.26 &  \cellcolor{mymax}2.13 &  \cellcolor{mymax}2.27 &  \cellcolor{mymax}2.39 &  \cellcolor{mymax}2.39 &  \cellcolor{mymax}2.77 &  \cellcolor{mymax}2.37 &  2.02 &  2.06 \\
  &    &  MTP (2:1:1)  &  \cellcolor{mymax}2.26 &  \cellcolor{mymax}2.15 &  \cellcolor{mymax}2.27 &  \cellcolor{mymax}2.40 &  \cellcolor{mymax}2.39 &  2.74 &  2.33 &  1.94 &  1.93 \\
  &    &  MTP (3:1:1)  &  \cellcolor{mymax}2.26 &  \cellcolor{mymax}2.15 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.40 &  \cellcolor{mymax}2.38 &  2.70 &  2.29 &  1.85 &  1.80 \\
  &    &  MTP (4:1:1)  &  \cellcolor{mymax}2.26 &  \cellcolor{mymax}2.15 &  \cellcolor{mymax}\secondbest{2.29} &  \cellcolor{mymax}2.40 &  \cellcolor{mymax}2.38 &  2.68 &  2.25 &  1.76 &  1.70 \\
  &    &  MTCP (1:1:1:1)  &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.16 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.41 &  \cellcolor{mymax}2.40 &  \cellcolor{mymax}\secondbest{2.78} &  \cellcolor{mymax}\secondbest{2.39} &  \cellcolor{mymax}\best{2.10} &  \cellcolor{mymax}\best{2.13} \\
  &    &  MTCP (2:1:1:1)  &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}\best{2.17} &  \cellcolor{mymax}\secondbest{2.29} &  \cellcolor{mymax}2.41 &  \cellcolor{mymax}2.40 &  2.76 &  \cellcolor{mymax}2.37 &  1.90 &  1.81 \\
  &    &  MTCP (3:1:1:1)  &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.16 &  \cellcolor{mymax}\secondbest{2.29} &  2.40 &  \cellcolor{mymax}2.40 &  2.75 &  2.35 &  1.79 &  1.70 \\
  &    &  MTCP (4:1:1:1)  &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.16 &  \cellcolor{mymax}\secondbest{2.29} &  2.40 &  \cellcolor{mymax}2.39 &  2.72 &  2.33 &  1.71 &  1.62 \\
\bottomrule
\end{tabular}
}
\caption{Block efficiency results of \ours{} for various weights. Results of IbED are \hlc[gray!15]{highlighted} when they show the best performance among all constituent methods (e.g., when MT performs best compared to M and T). The ensemble results are consistently \hlc[gray!15]{highlighted} across the weight variations.}
\label{tab:app_ensemble}
\end{table*}





\begin{table*}[h]
\centering
\sisetup{table-auto-round}
\resizebox{1.0\textwidth}{!}{% 
\begin{tabular}{lrl|ccccccc||cc}
\toprule
\multicolumn{3}{c|}{Draft Model} & \multicolumn{7}{c||}{\titlecap{\standard{} datasets}} & \multicolumn{2}{c}{\titlecap{\ood{} datasets}} \\%&$n=1$&$n=2$&$n=5$ \\
\cmidrule(lr){1-3}\cmidrule(lr){4-10}\cmidrule(lr){11-12}%\cmidrule(lr){12-12}\cmidrule(lr){13-13}\cmidrule(lr){14-14}
Type & Size & Method (Weights) & ChartQA \citep{masry2022chartqa} & TextVQA \citep{singh2019towards} & VQAv2 \citep{goyal2017making}& HBench \citep{guan2024hallusionbench}& Spot \citep{jhamtani2018learning}& WebQA \citep{chang2022webqa}& MB \citep{zhang2024magicbrush}& PSV \citep{li2019storygan}& VIST \citep{huang2016visual}\\
\midrule
\multirow{13}{*}{\shortstack[l]{LLaVA-1.5}}    &    \multirow{13}{*}{68M}    &    M    &  2.24 &  2.12 &  2.26 &  2.39 &  2.34 &  2.51 &  1.96 &  1.19 &  1.16 \\
    &        &    T    &  2.22 &  2.03 &  2.20 &  2.34 &  2.27 &  2.77 &  2.34 &  2.05 &  2.05 \\
    &        &    C    &  2.28 &  2.08 &  2.24 &  2.41 &  2.31 &  2.77 &  2.36 &  2.08 &  2.10 \\
    &        &    P    &  2.23 &  2.08 &  2.26 &  2.36 &  2.23 &  2.73 &  2.27 &  2.07 &  2.09 \\
     &          &     MTCP (1:1:1:1)     & \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.16} & \cellcolor{mymax}\secondbest{2.28} & \cellcolor{mymax}2.41 & \cellcolor{mymax}\best{2.40} & \cellcolor{mymax}2.78 & \cellcolor{mymax}2.39 & \cellcolor{mymax}2.10 & \cellcolor{mymax}2.13 \\
     &          &     MTCP (kld-1)   & \cellcolor{mymax}\best{2.29} & \cellcolor{mymax}\best{2.16} & \cellcolor{mymax}\secondbest{2.28} & \cellcolor{mymax}\best{2.42} & \cellcolor{mymax}\secondbest{2.39} &  \cellcolor{mymax}2.78 & \cellcolor{mymax}\best{2.42} & \cellcolor{mymax}\secondbest{2.12} &  \cellcolor{mymax}2.15 \\
     &          &     MTCP (kld-4)     & \cellcolor{mymax}\best{2.29} & \cellcolor{mymax}\best{2.16} & \cellcolor{mymax}\secondbest{2.28} & \cellcolor{mymax}\best{2.42} & \cellcolor{mymax}\secondbest{2.39} &  \cellcolor{mymax}2.78 & \cellcolor{mymax}\best{2.42} & \cellcolor{mymax}\secondbest{2.12} & \cellcolor{mymax}\best{2.17} \\
     &          &     MTCP (kld-16)     &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.16} & \cellcolor{mymax}\secondbest{2.28} &  \cellcolor{mymax}2.41 &  \cellcolor{mymax}2.38 & \cellcolor{mymax}\best{2.79} & \cellcolor{mymax}\best{2.42} & \cellcolor{mymax}\secondbest{2.12} & \cellcolor{mymax}\best{2.17} \\
     &          &     MTCP (kld-full)     &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.16} & \cellcolor{mymax}\secondbest{2.28} &  \cellcolor{mymax}2.41 & \cellcolor{mymax}\secondbest{2.39} & \cellcolor{mymax}\best{2.79} & \cellcolor{mymax}\best{2.42} & \cellcolor{mymax}\best{2.13} &  \cellcolor{mymax}2.16 \\
     &          &     MTCP (tvd-1)     & \cellcolor{mymax}\best{2.29} & \cellcolor{mymax}\best{2.16} & \cellcolor{mymax}\secondbest{2.28} & \cellcolor{mymax}\best{2.42} & \cellcolor{mymax}\secondbest{2.39} &  \cellcolor{mymax}2.78 &  \cellcolor{mymax}2.41 &  \cellcolor{mymax}2.11 &  \cellcolor{mymax}2.14 \\
     &          &     MTCP (tvd-4)     &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.16} & \cellcolor{mymax}\best{2.29} & \cellcolor{mymax}\best{2.42} & \cellcolor{mymax}\secondbest{2.39} &  \cellcolor{mymax}2.78 &  \cellcolor{mymax}2.41 & \cellcolor{mymax}\secondbest{2.12} &  \cellcolor{mymax}2.15 \\
     &          &     MTCP (tvd-16)     &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.16} & \cellcolor{mymax}\secondbest{2.28} &  \cellcolor{mymax}2.41 & \cellcolor{mymax}\secondbest{2.39} &  \cellcolor{mymax}2.78 & \cellcolor{mymax}\best{2.42} & \cellcolor{mymax}\secondbest{2.12} &  \cellcolor{mymax}2.15 \\
     &          &     MTCP (tvd-full)    &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.16} & \cellcolor{mymax}\secondbest{2.28} &  \cellcolor{mymax}2.41 & \cellcolor{mymax}\secondbest{2.39} & \cellcolor{mymax}\best{2.79} & \cellcolor{mymax}\best{2.42} & \cellcolor{mymax}\secondbest{2.12} &  \cellcolor{mymax}2.15 \\
\bottomrule
\end{tabular}
}
\caption{Block efficiency results of \ours{} with test-time adaptive ensemble weights. For example, MTCP (kld-4) indicates that the test-time adaptive ensemble weights were computed using KLD with a window size of 4. Results of IbED are \hlc[gray!15]{highlighted} when they show the best performance among all constituent methods (e.g., when MT performs best compared to M and T).
}
\label{tab:app_ensemble_test}
\end{table*}








\begin{table*}[h]
\centering
\sisetup{table-auto-round}
\resizebox{1.0\textwidth}{!}{% 
\begin{tabular}{lrl|ccccccc||cc}
\toprule
\multicolumn{3}{c|}{Draft Model} & \multicolumn{7}{c||}{\titlecap{\standard{} datasets}} & \multicolumn{2}{c}{\titlecap{\ood{} datasets}} \\%&$n=1$&$n=2$&$n=5$ \\
\cmidrule(lr){1-3}\cmidrule(lr){4-10}\cmidrule(lr){11-12}%\cmidrule(lr){12-12}\cmidrule(lr){13-13}\cmidrule(lr){14-14}
Type & Size & Method (Weights) & ChartQA \citep{masry2022chartqa} & TextVQA \citep{singh2019towards} & VQAv2 \citep{goyal2017making}& HBench \citep{guan2024hallusionbench}& Spot \citep{jhamtani2018learning}& WebQA \citep{chang2022webqa}& MB \citep{zhang2024magicbrush}& PSV \citep{li2019storygan}& VIST \citep{huang2016visual}\\
\midrule
\multirow{25}{*}{\shortstack[l]{LLaVA-1.5}}     &     \multirow{25}{*}{68M}     &     M     &  2.24 &  2.12 &  2.26 &  2.39 &  2.34 &  2.51 &  1.96 &  1.19 &  1.16 \\
     &          &     T     &  2.22 &  2.03 &  2.20 &  2.34 &  2.27 &  2.77 &  2.34 &  2.05 &  2.05 \\
     &          &     C     &  2.28 &  2.08 &  2.24 &  2.41 &  2.31 &  2.77 &  2.36 &  2.08 &  2.10 \\
     &          &     P     &  2.23 &  2.08 &  2.26 &  2.36 &  2.23 &  2.73 &  2.27 &  2.07 &  2.09 \\
       &              &       MTCP (1:1:1:1)       & \cellcolor{mymax}2.28 & \cellcolor{mymax}2.16 & \cellcolor{mymax}2.28 & \cellcolor{mymax}2.41 & \cellcolor{mymax}\best{2.40} & \cellcolor{mymax}2.78 & \cellcolor{mymax}2.39 & \cellcolor{mymax}2.10 & \cellcolor{mymax}2.13 \\
  &              &       MTCP (kld-1-0)    & 2.26 &  \cellcolor{mymax}2.14 &  \cellcolor{mymax}2.27 & \cellcolor{mymax}\best{2.42} & 2.31 & 2.72 & 2.33 & 2.04 & 2.07 \\
  &              &       MTCP (kld-1-0.25)    &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.16 &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.42} &  \cellcolor{mymax}2.37 & 2.76 &  \cellcolor{mymax}2.39 &  \cellcolor{mymax}2.10 &  \cellcolor{mymax}2.14 \\
  &              &       MTCP (kld-1-0.5)    & \cellcolor{mymax}\best{2.29} &  \cellcolor{mymax}2.16 & \cellcolor{mymax}\best{2.29} & \cellcolor{mymax}\best{2.42} &  \cellcolor{mymax}2.38 &  \cellcolor{mymax}2.78 &  \cellcolor{mymax}2.40 &  \cellcolor{mymax}2.12 &  \cellcolor{mymax}2.15 \\
  &              &       MTCP (kld-1-0.75)    & \cellcolor{mymax}\best{2.29} &  \cellcolor{mymax}2.16 &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.42} &  \cellcolor{mymax}2.38 &  \cellcolor{mymax}2.78 &  \cellcolor{mymax}2.40 &  \cellcolor{mymax}2.12 &  \cellcolor{mymax}2.15 \\
  &              &       MTCP (kld-1-1)    & \cellcolor{mymax}\best{2.29} &  \cellcolor{mymax}2.16 &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.42} & \cellcolor{mymax}\secondbest{2.39} &  \cellcolor{mymax}2.78 & \cellcolor{mymax}\best{2.42} &  \cellcolor{mymax}2.12 &  \cellcolor{mymax}2.15 \\
  &              &       MTCP (kld-4-0)    & 2.27 &  \cellcolor{mymax}2.12 &  \cellcolor{mymax}2.27 & 2.40 & 2.32 & 2.72 &  \cellcolor{mymax}2.37 &  \cellcolor{mymax}2.08 & 2.06 \\
  &              &       MTCP (kld-4-0.25)   &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.17} & \cellcolor{mymax}\best{2.29} & \cellcolor{mymax}\best{2.42} &  \cellcolor{mymax}2.37 & 2.76 &  \cellcolor{mymax}2.40 &  \cellcolor{mymax}2.12 &  \cellcolor{mymax}2.14 \\
  &              &       MTCP (kld-4-0.5)   &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.17} &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.42} & \cellcolor{mymax}\secondbest{2.39} &  \cellcolor{mymax}2.78 &  \cellcolor{mymax}2.40 &  \cellcolor{mymax}2.12 &  \cellcolor{mymax}2.16 \\
  &              &       MTCP (kld-4-0.75)   & \cellcolor{mymax}\best{2.29} & \cellcolor{mymax}\best{2.17} &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.42} & \cellcolor{mymax}\secondbest{2.39} &  \cellcolor{mymax}2.78 &  \cellcolor{mymax}2.40 &  \cellcolor{mymax}2.12 &  \cellcolor{mymax}2.15 \\
  &              &       MTCP (kld-4-1)    & \cellcolor{mymax}\best{2.29} &  \cellcolor{mymax}2.16 &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.42} & \cellcolor{mymax}\secondbest{2.39} &  \cellcolor{mymax}2.78 & \cellcolor{mymax}\best{2.42} &  \cellcolor{mymax}2.12 & \cellcolor{mymax}\best{2.17} \\
  &              &       MTCP (kld-16-0)   & 2.26 &  \cellcolor{mymax}2.15 &  \cellcolor{mymax}2.26 &  \cellcolor{mymax}2.41 & 2.31 & 2.72 &  \cellcolor{mymax}2.36 &  \cellcolor{mymax}2.08 & 2.08 \\
  &              &       MTCP (kld-16-0.25)   & \cellcolor{mymax}\best{2.29} & \cellcolor{mymax}\best{2.17} &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.42} &  \cellcolor{mymax}2.38 &  \cellcolor{mymax}2.78 &  \cellcolor{mymax}2.40 & \cellcolor{mymax}\best{2.13} &  \cellcolor{mymax}2.15 \\
  &              &       MTCP (kld-16-0.5)   & \cellcolor{mymax}\best{2.29} &  \cellcolor{mymax}2.16 &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.42} & \cellcolor{mymax}\secondbest{2.39} & \cellcolor{mymax}\best{2.79} &  \cellcolor{mymax}2.40 & \cellcolor{mymax}\best{2.13} &  \cellcolor{mymax}2.16 \\
  &              &       MTCP (kld-16-0.75)   &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.17} &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.41 & \cellcolor{mymax}\secondbest{2.39} & \cellcolor{mymax}\best{2.79} &  \cellcolor{mymax}2.40 & \cellcolor{mymax}\best{2.13} &  \cellcolor{mymax}2.16 \\
  &              &       MTCP (kld-16-1)    &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.16 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.41 &  \cellcolor{mymax}2.38 & \cellcolor{mymax}\best{2.79} & \cellcolor{mymax}\best{2.42} &  \cellcolor{mymax}2.12 & \cellcolor{mymax}\best{2.17} \\
  &              &       MTCP (kld-full-0)    & 2.25 &  \cellcolor{mymax}2.14 &  \cellcolor{mymax}2.27 &  \cellcolor{mymax}2.41 & 2.31 & 2.72 & 2.35 &  \cellcolor{mymax}2.08 & 2.08 \\
  &              &       MTCP (kld-full-0.25)    & \cellcolor{mymax}\best{2.29} &  \cellcolor{mymax}2.16 &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.42} &  \cellcolor{mymax}2.37 & \cellcolor{mymax}\best{2.79} &  \cellcolor{mymax}2.39 & \cellcolor{mymax}\best{2.13} &  \cellcolor{mymax}2.15 \\
  &              &       MTCP (kld-full-0.5)    &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.16 &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.42} & \cellcolor{mymax}\secondbest{2.39} & \cellcolor{mymax}\best{2.79} &  \cellcolor{mymax}2.40 & \cellcolor{mymax}\best{2.13} &  \cellcolor{mymax}2.16 \\
  &              &       MTCP (kld-full-0.75)    &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.17} &  \cellcolor{mymax}2.28 & \cellcolor{mymax}\best{2.42} & \cellcolor{mymax}\secondbest{2.39} & \cellcolor{mymax}\best{2.79} &  \cellcolor{mymax}2.40 & \cellcolor{mymax}\best{2.13} &  \cellcolor{mymax}2.16 \\
  &              &       MTCP (kld-full-1)    &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.16 &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.41 & \cellcolor{mymax}\secondbest{2.39} & \cellcolor{mymax}\best{2.79} & \cellcolor{mymax}\best{2.42} & \cellcolor{mymax}\best{2.13} &  \cellcolor{mymax}2.16 \\
\bottomrule
\end{tabular}
}
\caption{Block efficiency results of \ours{} with test-time adaptive ensemble weights. For example, MTCP (kld-4-0.5) indicates that the test-time adaptive ensemble weights were computed using KLD with a window size of 4 and a temperature of 0.5. Results of IbED are \hlc[gray!15]{highlighted} when they show the best performance among all constituent methods (e.g., when MT performs best compared to M and T).
}
\label{tab:app_ensemble_test2}
\end{table*}












\begin{table*}[h]
\centering
\sisetup{table-auto-round}
\resizebox{1.0\textwidth}{!}{% 
\begin{tabular}{lrl|ccccccc||cc}
\toprule
\multicolumn{3}{c|}{Draft Model} & \multicolumn{7}{c||}{\titlecap{\standard{} datasets}} & \multicolumn{2}{c}{\titlecap{\ood{} datasets}} \\%&$n=1$&$n=2$&$n=5$ \\
\cmidrule(lr){1-3}\cmidrule(lr){4-10}\cmidrule(lr){11-12}%\cmidrule(lr){12-12}\cmidrule(lr){13-13}\cmidrule(lr){14-14}
Type & Size & Method (Weights) & ChartQA \citep{masry2022chartqa} & TextVQA \citep{singh2019towards} & VQAv2 \citep{goyal2017making}& HBench \citep{guan2024hallusionbench}& Spot \citep{jhamtani2018learning}& WebQA \citep{chang2022webqa}& MB \citep{zhang2024magicbrush}& PSV \citep{li2019storygan}& VIST \citep{huang2016visual}\\
\midrule
\multirow{9}{*}{\shortstack[l]{LLaVA-1.5}}   &   \multirow{9}{*}{68M}   &   M   &  2.24 &  2.12 &  2.26 &  2.39 &  2.34 &  2.51 &  1.96 &  1.19 &  1.16 \\
   &      &   T   &  2.22 &  2.03 &  2.20 &  2.34 &  2.27 &  2.77 &  2.34 &  2.05 &  2.05 \\
   &      &   C   &  2.28 &  2.08 &  2.24 &  2.41 &  2.31 &  2.77 &  2.36 &  2.08 &  2.10 \\
   &      &   P   &  2.23 &  2.08 &  2.26 &  2.36 &  2.23 &  2.73 &  2.27 &  2.07 &  2.09 \\
   &      &   MTCP (1:1:1:1)   &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}\secondbest{2.16} &  \cellcolor{mymax}2.28 &  \cellcolor{mymax}2.41 &  \cellcolor{mymax}\secondbest{2.40} &  \cellcolor{mymax}2.78 &  \cellcolor{mymax}\secondbest{2.39} &  \cellcolor{mymax}\secondbest{2.10} &  \cellcolor{mymax}\secondbest{2.13} \\
   &      &   MTCP (logit-nll)  & \cellcolor{mymax} \best{2.29} & \cellcolor{mymax} \secondbest{2.16} & \cellcolor{mymax} \best{2.29} &  \cellcolor{mymax}\best{2.42} & \cellcolor{mymax} 2.39 &  \cellcolor{mymax}2.79 & \cellcolor{mymax} 2.38 & \cellcolor{mymax} 2.08 & \cellcolor{mymax} 2.11 \\
   &      &   MTCP (logit-kld)  & \cellcolor{mymax} \best{2.29} & \cellcolor{mymax} \secondbest{2.16} & \cellcolor{mymax} 2.27 &  \cellcolor{mymax}2.41 & \cellcolor{mymax} 2.39 & \cellcolor{mymax} \best{2.80} & \cellcolor{mymax} 2.38 & \cellcolor{mymax} 2.09 &  \cellcolor{mymax}2.12 \\
   &      &   MTCP (probability-nll)  & \cellcolor{mymax} \best{2.29} & \cellcolor{mymax} 2.14 &  \cellcolor{mymax}2.26 & \cellcolor{mymax} \best{2.42} &  2.31 &  \cellcolor{mymax}2.79 & \cellcolor{mymax} \secondbest{2.39} &  1.52 &  1.59 \\
   &      &   MTCP (probability-kld)  & \cellcolor{mymax} \best{2.29} & \cellcolor{mymax} \best{2.18} & \cellcolor{mymax} \best{2.29} & \cellcolor{mymax} 2.41 &  \cellcolor{mymax}\best{2.42} &  \cellcolor{mymax}\best{2.80} & \cellcolor{mymax} \best{2.40} &  \cellcolor{mymax}\best{2.13} & \cellcolor{mymax} \best{2.15} \\
\bottomrule
\end{tabular}
}
\caption{Block efficiency results of \ours{} with learnable ensemble weights. Results of IbED are \hlc[gray!15]{highlighted} when they show the best performance among all constituent methods (e.g., when MT performs best compared to M and T). MTCP (probability-kld) consistently demonstrates the best performance among the various ensemble weights tested.
}
\label{tab:app_ensemble2}
\end{table*}

\begin{table*}[h]
\centering
\sisetup{table-auto-round}
\resizebox{1.0\textwidth}{!}{% 
\begin{tabular}{lrl|ccccccc||cc}
\toprule
\multicolumn{3}{c|}{Draft Model} & \multicolumn{7}{c||}{\titlecap{\standard{} datasets}} & \multicolumn{2}{c}{\titlecap{\ood{} datasets}} \\%&$n=1$&$n=2$&$n=5$ \\
\cmidrule(lr){1-3}\cmidrule(lr){4-10}\cmidrule(lr){11-12}%\cmidrule(lr){12-12}\cmidrule(lr){13-13}\cmidrule(lr){14-14}
Type & Size & Method & ChartQA \citep{masry2022chartqa} & TextVQA \citep{singh2019towards} & VQAv2 \citep{goyal2017making}& HBench \citep{guan2024hallusionbench}& Spot \citep{jhamtani2018learning}& WebQA \citep{chang2022webqa}& MB \citep{zhang2024magicbrush}& PSV \citep{li2019storygan}& VIST \citep{huang2016visual}\\
\midrule

\multirow{4}{*}{\shortstack[l]{LLaVA-1.5}} & \multirow{4}{*}{68M}
    & M & 0.392 & 0.502 & 0.577 & 0.348 & 0.393 & 0.178 & 0.117 & 0.007 & 0.005 \\
 &  & T & 0.316 & 0.305 & 0.341 & 0.307 & 0.227 & 0.500 & 0.365 & 0.215 & 0.281 \\
 &  & C & 0.258 & 0.157 & 0.079 & 0.336 & 0.297 & 0.146 & 0.314 & 0.224 & 0.260 \\
 &  & P & 0.034 & 0.036 & 0.003 & 0.009 & 0.083 & 0.176 & 0.204 & 0.554 & 0.454 \\


\bottomrule
\end{tabular}
}
%\vspace{-4pt}
\captionsetup{skip=5pt}
\caption{Learned ensemble weights for MTCP (probability-kld) in \cref{tab:app_ensemble2}. Different weights are assigned to each of the M, T, C, and P, depending on the dataset characteristics. The weights are normalized using the softmax function.}
% \caption{\ba{Learned ensemble weights for MTCP (probability-kld) in \cref{tab:app_ensemble2}. Different weights are assigned to each of the M, T, C, nd P, depending on the dataset characteristics.}}
\label{tab:app_learnable_ensemble}
\end{table*}









\begin{comment}

\begin{table*}[h]
\centering
\sisetup{table-auto-round}
\resizebox{1.0\textwidth}{!}{% 
\begin{tabular}{lll|rrrrrrrr|rrr}
\toprule
\multicolumn{3}{c|}{Target / Draft} & \multicolumn{4}{c}{$n=1$} & \multicolumn{2}{c}{$n=2$} & \multicolumn{2}{c}{$n=5$} &$n=1$&$n=2$&$n=5$ \\
\cmidrule(lr){1-3}\cmidrule(lr){4-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-12}\cmidrule(lr){13-13}\cmidrule(lr){14-14}
Model & Size & Method  & ChartQA & TextVQA & VQAv2 & Hallusion & Spot & IEdit & PororoSV & VIST &Avg. &Avg. &Avg.\\
\midrule
\multirow{20}{*}{\shortstack[l]{LLaVA 1.5}} & \multirow{20}{*}{7B / 68M} & M & 2.24 & 2.12 & 2.26 & 2.39 & 2.34 & 2.19 & 1.19 & 1.16 & 2.25 & 2.26 & 1.17 \\
 &  & T & 2.22 & 2.03 & 2.20 & 2.34 & 2.27 & 2.23 & 2.05 & 2.05 & 2.20 & 2.25 & 2.05 \\
 &  & C & 2.28 & 2.08 & 2.24 & \cellcolor{mysilver}2.41 & 2.31 & 2.29 & \cellcolor{mygold}2.08 & \cellcolor{mygold}2.10 & 2.25 & 2.30 & \cellcolor{mygold}2.09 \\
 &  & P & 2.23 & 2.08 & 2.26 & 2.36 & 2.23 & 2.22 & \cellcolor{mysilver}2.07 & \cellcolor{mysilver}2.09 & 2.23 & 2.23 & \cellcolor{mysilver}2.08 \\
 &  & \textbf{MT (1)} & 2.26 & 2.13 & 2.27 & 2.39 & \cellcolor{mysilver}2.40 & 2.31 & 1.94 & 1.91 & 2.26 & \cellcolor{mysilver}2.35 & 1.92 \\
 &  & \textbf{MT (2)} & 2.26 & 2.13 & \cellcolor{mysilver}2.29 & 2.39 & \cellcolor{mysilver}2.40 & 2.29 & 1.76 & 1.69 & 2.27 & 2.34 & 1.73 \\
 &  & \textbf{MT (3)} & 2.26 & 2.13 & 2.28 & 2.40 & 2.38 & 2.28 & 1.63 & 1.54 & 2.27 & 2.33 & 1.58 \\
 &  & \textbf{MT (4)} & 2.26 & 2.14 & 2.28 & 2.40 & 2.36 & 2.26 & 1.54 & 1.45 & 2.27 & 2.31 & 1.50 \\
 &  & \textbf{MC (1)} & \cellcolor{mygold}2.30 & \cellcolor{mygold}2.17 & \cellcolor{mysilver}2.29 & \cellcolor{mygold}2.42 & 2.39 & \cellcolor{mysilver}2.32 & 1.99 & 1.93 & \cellcolor{mygold}2.29 & \cellcolor{mysilver}2.35 & 1.96 \\
 &  & \textbf{MC (2)} & \cellcolor{mygold}2.30 & \cellcolor{mygold}2.17 & \cellcolor{mygold}2.30 & \cellcolor{mysilver}2.41 & 2.39 & 2.31 & 1.80 & 1.71 & \cellcolor{mygold}2.29 & \cellcolor{mysilver}2.35 & 1.75 \\
 &  & \textbf{MC (3)} & \cellcolor{mysilver}2.29 & \cellcolor{mysilver}2.16 & \cellcolor{mysilver}2.29 & 2.40 & 2.38 & 2.29 & 1.66 & 1.56 & \cellcolor{mygold}2.29 & 2.33 & 1.61 \\
 &  & \textbf{MC (4)} & 2.28 & \cellcolor{mysilver}2.16 & \cellcolor{mysilver}2.29 & 2.40 & 2.37 & 2.28 & 1.56 & 1.46 & \cellcolor{mysilver}2.28 & 2.33 & 1.51 \\
 &  & \textbf{MTC (1)} & \cellcolor{mysilver}2.29 & 2.15 & 2.28 & \cellcolor{mysilver}2.41 & \cellcolor{mygold}2.41 & 2.30 & \cellcolor{mygold}2.08 & 2.06 & \cellcolor{mysilver}2.28 & \cellcolor{mysilver}2.35 & 2.07 \\
 &  & \textbf{MTC (2)} & \cellcolor{mysilver}2.29 & \cellcolor{mygold}2.17 & \cellcolor{mysilver}2.29 & \cellcolor{mygold}2.42 & \cellcolor{mygold}2.41 & 2.30 & 1.99 & 1.96 & \cellcolor{mygold}2.29 & \cellcolor{mysilver}2.35 & 1.98 \\
 &  & \textbf{MTC (3)} & 2.28 & \cellcolor{mygold}2.17 & \cellcolor{mysilver}2.29 & \cellcolor{mysilver}2.41 & 2.39 & 2.29 & 1.90 & 1.83 & \cellcolor{mygold}2.29 & 2.34 & 1.86 \\
 &  & \textbf{MTC (4)} & 2.28 & \cellcolor{mysilver}2.16 & \cellcolor{mysilver}2.29 & 2.40 & 2.39 & 2.28 & 1.80 & 1.71 & \cellcolor{mysilver}2.28 & 2.33 & 1.75 \\
 &  & \textbf{MTCP (1)} & \cellcolor{mysilver}2.29 & \cellcolor{mygold}2.17 & \cellcolor{mysilver}2.29 & \cellcolor{mygold}2.42 & \cellcolor{mygold}2.41 & \cellcolor{mygold}2.33 & 1.99 & 1.93 & \cellcolor{mygold}2.29 & \cellcolor{mygold}2.37 & 1.96 \\
 &  & \textbf{MTCP (2)} & 2.28 & \cellcolor{mygold}2.17 & \cellcolor{mysilver}2.29 & \cellcolor{mysilver}2.41 & \cellcolor{mysilver}2.40 & 2.31 & 1.90 & 1.81 & \cellcolor{mygold}2.29 & \cellcolor{mysilver}2.35 & 1.85 \\
 &  & \textbf{MTCP (3)} & 2.28 & \cellcolor{mysilver}2.16 & \cellcolor{mysilver}2.29 & 2.40 & \cellcolor{mysilver}2.40 & 2.31 & 1.79 & 1.70 & \cellcolor{mysilver}2.28 & \cellcolor{mysilver}2.35 & 1.75 \\
 &  & \textbf{MTCP (4)} & 2.28 & \cellcolor{mysilver}2.16 & \cellcolor{mysilver}2.29 & 2.40 & 2.39 & 2.29 & 1.71 & 1.62 & \cellcolor{mysilver}2.28 & 2.34 & 1.67 \\
\bottomrule
\end{tabular}
}
\caption{Block efficiency results of ensemble drafting for various weights.}
\label{tab:app_ensemble}
\end{table*}
    
\end{comment}
